Reachability in Controlled Markovian Quantum Systems: An Operator-Theoretic Approach

In quantum systems theory one of the fundamental problems boils down to: Given an initial state, which final states can be reached by the dynamic system in question? Formulated in the framework of bilinear control systems, the evolution shall be governed by an inevitable Hamiltonian drift term, finitely many control Hamiltonians allowing for (at least) piecewise constant control amplitudes, plus a (possibly bang-bang switchable) noise term in Kossakowski-Lindblad form. Now assuming switchable coupling of finite-dimensional systems to a thermal bath of arbitrary temperature, the core problem of reachability boils down to studying points in the standard simplex amenable to two types of controls that can be used interleaved: Permutations within the simplex, and contractions by a dissipative one-parameter semigroup. We illustrate how the solutions of the core problem pertain to the reachable set of the original controlled Markovian quantum system. This allows us to show that for global as well as local switchable coupling to a temperature-zero bath one can generate every quantum state from every initial state up to arbitrary precision. Moreover we present an inclusion for non-zero temperatures as a consequence of our results on d-majorization. Then we consider infinite-dimensional open quantum-dynamical systems following a unital Kossakowski-Lindblad master equation extended by controls. Here the drift Hamiltonian can be arbitrary, the finitely many control Hamiltonians are bounded, and the switchable noise term is generated by a single compact normal operator. Via new majorization results of ours, we show that such bilinear quantum control systems allow to approximately reach any target state majorized by the initial one, as up to now only has been known in finite-dimensional analogues.

==> pages/abstract.tex <==
\chapter*{Abstract}


In quantum systems theory one of the fundamental problems boils down to: given an initial state, which
final states can be reached by the dynamic system in question? Formulated in the framework of bilinear control systems, the evolution shall be governed by an inevitable Hamiltonian drift term, finitely many control Hamiltonians allowing for (at least) 
piecewise constant control amplitudes plus a bang-bang switchable noise 
term in Kossakowski-Lindblad form. We present results for reachable sets of such coherently controllable open 
quantum systems with switchable coupling of the following two models:

First we consider switchable coupling of finite-dimensional systems to a thermal bath of arbitrary temperature.
The core problem boils down to studying points in the standard simplex amenable to two types 
of controls that can be used interleaved:
\begin{itemize}
\item[(i)] permutations within the simplex,
\item[(ii)] contractions by a dissipative one-parameter semigroup.
\end{itemize}
We illustrate how the solutions of the core problem pertain to the reachable set of the original
controlled Markovian quantum system. This allows us to show that for global as well as local switchable coupling to a temperature-zero bath one can (approximately) generate every quantum state from every initial state. Moreover we present an inclusion
for non-zero temperature as a consequence of recent results of ours regarding $d$-majorization. 

Then we consider infinite-dimensional 
open quantum dynamical systems following a unital Kossakowski-Lindblad master equation extended
by controls. Here the drift Hamiltonian can be arbitrary, the finitely many control Hamiltonians are bounded and the noise term is generated by a single compact normal operator. Generalizing standard majorization results from finite to infinite 
dimensions, we show that such bilinear quantum control systems allow to approximately reach
any target state majorized by the initial one as up to now only has been known in finite dimensional
analogues.


\newpage\null\thispagestyle{empty}\newpage
\chapter*{Zusammenfassung}

{\Large Titel: Erreichbarkeit in Kontrollierten Markovschen Quantensystemen: Ein Operatortheoretischer Ansatz}\vspace*{15pt}

\noindent Eines der fundamentalen Probleme der Quantensystemstheorie lautet: f{\"u}r einen gegebenen Anfangszustand, welche Endzust{\"a}nde k{\"o}nnen innerhalb eines dynamischen Systems erreicht werden? Formuliert im Rahmen bilinearer Kontrolltheorie wird die Zeitentwicklung des Systems durch einen unvermeidbaren Hamiltonschen Drift, endlich viele Kontroll-Hamiltonians mit mindestens st{\"u}ckweise konstanten Kontrollen, und ``Bang-Bang'' schaltbarer Kopplung an die Systemsumgebung in Kossakowski-Lindblad-Form beschrieben. Wir pr{\"a}sentieren Ergebnisse f{\"u}r Erreichbarkeitsmengen solcher koh{\"a}rent kontrollierbaren offenen Quantensysteme mit schaltbarer Kopplung f{\"u}r die folgenden zwei Modelle:

Zuerst untersuchen wir schaltbare Kopplung beliebiger endlichdimensionaler Systeme an ein thermales Bad endlicher Temperatur. Das Kernproblem l{\"a}uft auf die Betrachung von Punkten im Standard-Simplex hinaus, welche den folgenden zwei abwechselnd einsetzbaren Kontrollen ausgesetzt sind:
\begin{itemize}
\item[(i)] Permutationen im Simplex,
\item[(ii)] Kontraktionen durch eine dissipative Ein-Parameter Halbgruppe.
\end{itemize}
Wir zeigen wie sich L{\"o}sungen des Kernproblems auf die Erreichbarkeitsmenge des urspr{\"u}nglichen kontrollierten Markovschen Quantensystems {\"u}bertragen. Dies erlaubt uns zu zeigen, dass man f{\"u}r globale, sowie lokale schaltbare Kopplung an ein Bad der Temperatur Null jeden Zustand von jedem Anfangszustand aus (approximativ) erreichen kann. 
Au{\ss}erdem pr{\"a}sentieren wir eine Obermenge f{\"u}r Temperatur ungleich Null, welche eine Konsequenz unserer neuen Ergebnisse bez{\"u}glich $d$-Majorisierung.

Als zweites untersuchen wir unendlichdimensionale offene quanten-dynamische Systeme welche einer unitalen Kossakowski-Lindblad Mastergleichung, erweitert durch Kontrollen, folgen. Der Hamiltonsche Drift kann beliebig sein, die endlich vielen Kontrollhamiltonians sind beschr{\"a}nkt und die Kopplung an die Umgebung wird von einem einzigen, kompakten, normalen Operator erzeugt. Durch Verallgemeinerung von Standardergebnissen bez{\"u}glich Majorisierung von endlichen zu unendlichen Dimensionen zeigen wir, dass innerhalb solcher bilinearen Quantenkontrollsysteme jeder Zustand approximativ erreicht werden kann, welcher vom Anfangszustand majorisiert wird -- ein Ergebnis, das bisher nur in endlichen Dimensionen bekannt war.
